CollComm: Enabling Efficient Collective Quantum Communication Based on EPR buffering

The noisy and lengthy nature of quantum communication hinders the development of distributed quantum computing. The inefficient design of existing compilers for distributed quantum computing worsens the situation. Previous compilation frameworks couple communication hardware with the implementation of expensive remote gates. However, we discover that the efficiency of quantum communication, especially collective communication, can be significantly boosted by decoupling communication resources from remote operations, that is, the communication hardware would be used only for preparing remote entanglement, and the computational hardware, the component used to store program information, would be used for conducting remote gates. Based on the observation, we develop a compiler framework to optimize the collective communication happening in distributed quantum programs. In this framework, we decouple the communication preparation process in communication hardware from the remote gates conducted in computational hardware by buffering EPR pairs generated by communication hardware in qubits of the computational hardware. Experimental results show that the proposed framework can halve the communication cost of various distributed quantum programs, compared to state-of-the-art compilers for distributed quantum computing.

==> old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% new DQC compiler papers
% Divide and Conquer for Combinatorial Optimization and Distributed Quantum Computation
% Optimized Quantum Circuit Partitioning
% Reordering and Partitioning of Distributed Quantum Circuits
% Distribution of Quantum Circuits Over General Quantum Networks: execution memory which is to store communication qubit (more like communication qubits, the maximal links can be established among nodes), but not to buffer EPR pairs;
% A general protocol for distributed quantum gates
% Distributed Quantum Computation Assisted by Remote Toffoli Gate
% Automated distribution of quantum circuits via hypergraph partitioning, includes a discussion about distributed quantum architecture, very nice!
% Efficient Distribution of Quantum Circuits
% A dynamic programming approach for distributing quantum circuits by bipartite graphs
% Efficient distributed quantum computing
% Optimizing Teleportation Cost in Distributed Quantum Circuits
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% other papers interesting
% A quantum router architecture for high-fidelity entanglement flows in quantum networks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering
\caption{The compilation results of {\frameworkName} on benchmark programs. %\todo{check \#qubit and \#gate.}
}
\label{tab:benchmark}
\def\nsize {1.75cm}
\resizebox{0.98\textwidth}{!}{
\renewcommand*{\arraystretch}{1.3}
\begin{tabular}{|p{1.0cm}|p{\nsize}|p{0.7cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{1.2cm}|p{0.9cm}|p{0.8cm}|p{1.2cm}|p{0.8cm}|p{1.cm}|} 
    \hline
    \multirow{2}{*}{Type} & \multirow{2}{*}{Name} & \multirow{2}{*}{\# qubit} & \multirow{2}{*}{\# gate} & \multirow{2}{*}{\# CX} & \multicolumn{5}{c|}{QuComm} & \multicolumn{4}{c|}{Compared to AutoComm} \\ 
    \cline{6-14}
     &  &  &  &  & \# node & AVG CB \#q & \# EPR & \# CROSS EPR & Latency & EPR-DEC & CROSS-EPR-DEC & LAT-DEC & FD-INC \\ 
    \hline
    \multirow{9}{1cm}{Building Blocks} & \multirow{3}{\nsize}{Multi-Controlled Gate (MCTR)} & 100 & 10640 & 4560 & 3 & 1.333 & 2 & 0 & 2521.3 & 0.6 & 0 & 0.045 & 0.109 \\ 
    \cline{3-14}
     &  & 200 & 21840 & 9360 & 6 & 1.667 & 5 & 2 & 2547.7 & 0.8 & 0.333 & 0.263 & 1.195 \\ 
    \cline{3-14}
     &  & 300 & 33040 & 14160 & 8 & 1.75 & 7 & 4 & 2917.3 & 0.811 & 0.636 & 0.398 & 4.499 \\ 
    \cline{2-14}
     & \multirow{3}{\nsize}{Ripple-Carry Adder (RCA)} & 100 & 1569 & 785 & 3 & 1.333 & 4 & 0 & 872.6 & 0.5 & 0 & 0.081 & 0.139 \\ 
    \cline{3-14}
     &  & 200 & 3169 & 1585 & 6 & 1.667 & 10 & 2 & 1775.8 & 0.375 & 0.5 & 0.151 & 0.470 \\ 
    \cline{3-14}
     &  & 300 & 4769 & 2385 & 8 & 1.75 & 14 & 2 & 2664.6 & 0.5 & 0.5 & 0.143 & 0.900 \\ 
    \cline{2-14}
     & \multirow{3}{\nsize}{Cat-State Preparation (CSP)} & 100 & 100 & 99 & 3 & 0.333 & 2 & 0 & 63.4 & 0 & 0 & 0.427 & 0.005 \\ 
    \cline{3-14}
     &  & 200 & 200 & 199 & 6 & 0.667 & 5 & 1 & 158.4 & -0.25 & 0 & 0.547 & -0.011 \\ 
    \cline{3-14}
     &  & 300 & 300 & 299 & 8 & 0.75 & 7 & 1 & 164.4 & 0 & 0.75 & 0.792 & 0.374 \\ 
    \hline
    \multirow{9}{1cm}{Real World Appli-cations} & \multirow{3}{\nsize}{Quantum Fourier Transformation (QFT)} & 100 & 19900 & 9900 & 3 & 6 & 98 & 0 & 3903.9 & -0.225 & 0 & 0.638 & 0.148 \\ 
    \cline{3-14}
     &  & 200 & 79800 & 39800 & 6 & 6 & 492 & 64 & 9790.5 & -0.23 & 0.6 & 0.772 & $>>1e^3$ \\ 
    \cline{3-14}
     &  & 300 & 179700 & 89700 & 8 & 2.5 & 1058 & 152 & 38822.2 & -0.080 & 0.729 & 0.913 & $>>1e^9$ \\ 
    \cline{2-14}
     & \multirow{3}{\nsize}{Bernstein Vazirani (BV)} & 100 & 209 & 69 & 3 & 0 & 1 & 0 & 55.3 & 0 & 0 & 0.002 & 0.000 \\ 
    \cline{3-14}
     &  & 200 & 419 & 139 & 5 & 0.333 & 3 & 0 & 73.4 & 0 & 0 & 0.583 & 0.010 \\ 
    \cline{3-14}
     &  & 300 & 629 & 209 & 8 & 0.5 & 5 & 1 & 160.4 & 0 & 0.5 & 0.661 & 0.123 \\ 
    \cline{2-14}
     & \multirow{3}{\nsize}{QAOA} & 100 & 5940 & 3960 & 3 & 4 & 60 & 0 & 1323.0 & 0 & 0 & 0.476 & 0.128 \\ 
    \cline{3-14}
     &  & 200 & 16200 & 10800 & 6 & 4 & 300 & 40 & 3545.0 & 0 & 0.75 & 0.726 & $>>1e^3$ \\ 
    \cline{3-14}
     &  & 300 & 26940 & 17960 & 8 & 2.5 & 560 & 80 & 8294.0 & 0 & 0.75 & 0.958 & $>>1e^9$ \\
    \hline
\end{tabular}
}
\end{table*}


\clearpage
\section{\frameworkNameSpace IR}

In this section, we introduce a compact IR of quantum communications and present an analysis of communication patterns in distributed quantum programs based on the proposed IR.


\iffalse
\subsection{Syntax and Semantics}

The objective of the new IR is to maintain high-level  information of quantum communications. We introduce its syntax and semantics as following:

% time ordering


\paragraph{Syntax:}
\todo{rephrase this paragraph: 
Copy paulihedral.
}

\paragraph{Semantics:} \todo{provide some insight}.

Our IR is mainly designed for internal compilation passes, but we also provide interface for users to inject custom IR manually into the compiler pass.
\fi

\subsection{State and Operation}

The state of the \frameworkNameSpace IR is defined by a set of adjacency matrices that represent quantum communications. Figure~\ref{} shows the IR generated from the Toffoli gate. 
The locations of involved qubits is defined by the tuple (rank, index). Here rank refers to the quantum computing routine on each node. Each rank actually has two buffers: one for communication and the other one for computation.
We omit the qubits used for communication here as they are being handled by the communication buffer manager automatically in Section~\ref{}.
% Each rank has two kind of quantum buffers: one for communication and the other one for computation. The size of each buffer may be dynamically changed by design.
For simplicity, we adopt the graphic representation of the adjacency matrix rather than its numeric form in the rest of the paper.

\subsection{Compiling to \frameworkNameSpace IR}

\subsection{Collective Communication Patterns and optimizations}

\paragraph{Communication Merging}

\paragraph{Communication Splitting}

\section{Extend to General DQC Topology}

In the section, we extend collective communication optimizations to DQC systems with a complicate network topology.

\subsection{The Hierarchical Network Topology}



\todo{may move it to the challenge section.}
We consider a hierarchical network model where compute nodes forming  clusters representing short-range networks (e.g. local area network or on-chip network) and clusters forming a long-range quantum network resembling quantum internet. Figure~\ref{fig:netmodel} depicts the topology of an example hierarchical network.

\begin{table}[h]
\caption{Quantitative data of operations in DQC (from~\cite{isailovic2006interconnection, Valivarthi2020TeleportationST, Rakonjac2021EntanglementBA, correa2018ultra}, with latencies normalized to CX counts).} 
\label{tab:netdata}
\centering
\scriptsize
\renewcommand*{\arraystretch}{1}
\begin{tabular}{|l|c|l|l|}
\hline
Operation & Variable Name & Latency & Fidelity \\ \hline
Single-qubit gates & $t_{1q}$ & $\sim$ 0.1 CX & 99.99\% \\ \hline
CX and CZ gates & $t_{2q}$ & 1 CX & 99.77\% \\ \hline
Measure & $t_{ms}$ & 5 CX  & - \\ \hline
Intra-cluster EPR preparation %\footnotemark 
& $t_{inep}$ & $\sim$ 12 CX & $\sim$ 98\%  \\ \hline
% EPR purification & $t_{pf}$ & $\sim$ 6 CX \\ \hline
Intra-cluster classical comm & $t_{incb}$ & $\sim$ 1 CX & - \\ \hline
Inter-cluster EPR preparation %\footnotemark 
& $t_{itep}$ & $\ge 10^3$ CX & $\sim$ 90\%  \\ \hline
% EPR purification & $t_{pf}$ & $\sim$ 6 CX \\ \hline
Inter-cluster classical comm & $t_{itcb}$ & $\ge 10^3$ CX & - \\ \hline
\end{tabular}
\end{table}

There are two types of quantum communications happening in the hierarchical network: intra-cluster communication and inter-cluster communication. Inter-cluster communication is typically more noisy and time-consuming than intra-cluster communication, as shown in Table~\ref{tab:netdata}. Thus, different strategies are needed to optimize intra-cluster and inter-cluster communication efficiently.

In the section, we only focus on the hierarchical network model with two levels. Networks with more levels can be handled by apply optimizations in this section recursively.

\subsection{Intra-cluster communication optimization}

For optimizing the intra-cluster communication, we should reduce the overall communication footprint of the collective operation, instead of simply shortening paths between any two communication endpoints.
% Intra-cluster communication should be optimized by optimizing the overall communication footprint of collective operations.
% reusing communication endpoints for communication relay. 
To demonstrates the difference between these two optimization targets, 
consider the example in Figure~\ref{fig:intraexam} where we are multi-casting $q_1$ to nodes B, D, and E. 
The shortest path for establishing the cat-state on $q_1$ and $q_4$ is by $q_1 \to q_3 \to q_4$ as it has the highest overall fidelity along the path. However, this shortest path does not lead to the minimal overall fingerprint of the multi-cast operation. 
As shown in Figure~\ref{fig:intraexam}, using the blue paths $q_1 \to q_2 \to q_4$, we can establish the cat-state on $\{q_1, q_2, q_4\}$ with only two quantum communications. In contrast, using the path $q_1 \to q_3 \to q_4$ would invoke one more quantum communication to build the cat-state on $\{q_1, q_2, q_4\}$ and surprisingly degrade the overall fidelity of the multi-cast operation.

By inspecting the communication patterns in distributed quantum programs, we discover that the optimization of intra-cluster collective communications falls into two cases:
\begin{enumerate}
    \item Multi-cast, multi-reduce, broadcast, reduce, and parity checking.
    \item Qubit passing in TP-Comm blocks and edge traversing on graphs.
\end{enumerate}

\paragraph{Observation 1:}
The problem of optimizing the footprint of collective communications in the first category can be formulated as the minimum spanning tree (MST) problem.  \todo{provide details.}

\paragraph{Observation 2:} The problem of optimizing the footprint of collective communications in the second category can be formulated as the travelling salesman problem (TSP) problem. \todo{provide details.}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figure/intra_exam.pdf}
    \caption{The data flow for broadcasting $q_1$ to node B, D, and E. Directed edges means to establish cat-state between the starting qubit and the ending qubit. Communication qubits omitted for simplicity.
    The weight on inter-node edges represents the fidelity of the channel (i.e. EPR pair). }
    \label{fig:intraexam}
\end{figure}

% Intra-cluster collective communication with other patterns can be addressed in a similar way. 

% We abstract the above procedure into the tree-based intra-cluster router in Algorithm~\ref{}.

We would then invoke associated solvers to address intra-cluster collective communication optimization problem. The goal is to boost the fidelity and minimize the latency.

\subsection{Inter-cluster communication optimization}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/inter_exam.pdf}
    \caption{Broadcasting $q_1$ to node B, C, and $q_2$ to node D. Assuming  only one current available communication channel between node A and node B. }
    \label{fig:interexam}
\end{figure}

We cannot simply apply the intra-cluster communication optimization to the inter-cluster case as 
it is much harder and more time-consuming to establish a communication channel between nodes in different cluster than nodes in the same cluster. For example in Figure~\ref{fig:interexam}, we are broadcasting $q_1$ to nodes B, C and $q_2$ to node D, respectively. There are two ways to fulfill these inter-cluster communication, as shown in Figure~\ref{fig:interexam}(a)(b). The communication path in Figure~\ref{fig:interexam}(a) is simply generated by solving the MST problem. 
The shortcoming of this communication schedule is that
we have to wait for a long communication preparation time for broadcasting $q_2$ to node B
as the only available communication channel between node A and B is consumed previously by broadcasting $q_1$.
To reduce the overall communication latency and improve the information throughput, we propose to use the communication schedule shown in Figure~\ref{fig:interexam}(b). The key idea behind Figure~\ref{fig:interexam}(b) is that we should exploit all available inter-cluster channels for data transfer, instead of sticking to the schedule generated by the intra-cluster communication optimizer. 

\todo{ provide the most essential reason}
The reason for this design is that the communication resource between intra-cluster nodes is more abundant and easier to prepare. It's not often to have communication resources used up, equipping with the communication buffer. In contrast, the number of inter-cluster communication channel is limited and takes a long time to prepare. Unnecessary stalling would greatly degrade the communication throughput, invalidating the potential fidelity gain by stalling the communication.

Overall, our algorithms to optimize the inter-cluster communication is summarized in Algorithm~\ref{}. It modifies the Algorithm~\ref{} to use any available inter-cluster communication channel to improve the throughput.

\section{Communication Buffer Optimization}

In this section, we introduce the optimization of the communication buffer to reduce the overall latency induced by quantum communication and achieve a balance between communication resources and computational resources. The input of the buffer optimization pass is the distributed quantum programs with all quantum communication footprints decided and the output is a schedule of communication resource preparation in the communication buffer.

\subsection{Buffer Allocation Optimization}

Buffer size estimation:
limited, adaptive, full. Copy PCCS.

\subsection{EPR Entanglement Generation Optimization}

% \subsection{Communication buffer adaptation}

Assume a more general connectivity model. Communication buffer relies on the compiled program flow and thus should be the last optimization pass.



% reduce does not care about the order of operations.
% Parity checking in UCCSD.
% reduce in BV and Grover.
% % Broadcast in QFT.
% The optimization of broadcast and reduce is similar. 
% The optimization of successive TP-Comm connection.
% Random graph in QAOA.
% Multi-cast in multi-controlled gates.
